A Class of Prediction-Correction Methods for Time-Varying Convex Optimization

This paper considers unconstrained convex optimization problems with time-varying objective functions. We propose algorithms with a discrete time-sampling scheme to find and track the solution trajectory based on prediction and correction steps, while sampling the problem data at a constant rate of $1/h$, where $h$ is the length of the sampling interval. The prediction step is derived by analyzing the iso-residual dynamics of the optimality conditions. The correction step adjusts for the distance between the current prediction and the optimizer at each time step, and consists either of one or multiple gradient steps or Newton steps, which respectively correspond to the gradient trajectory tracking (GTT) or Newton trajectory tracking (NTT) algorithms. Under suitable conditions, we establish that the asymptotic error incurred by both proposed methods behaves as $O(h^2)$, and in some cases as $O(h^4)$, which outperforms the state-of-the-art error bound of $O(h)$ for correction-only methods in the gradient-correction step. Moreover, when the characteristics of the objective function variation are not available, we propose approximate gradient and Newton tracking algorithms (AGT and ANT, respectively) that still attain these asymptotical error bounds. Numerical simulations demonstrate the practical utility of the proposed methods and that they improve upon existing techniques by several orders of magnitude.

==> Algorithm.tex <==
% !TEX root = TimeVarying_part1.tex
\section{Centralized algorithm}\label{sec:centr}

We first focus on centralized algorithms, i.e., algorithms that assume that the computations are performed by a unique computing entity. In order to converge to the solution trajectory $\x^*(t)$, we will generate a sequence of near optimal decision variables $\{\x_k\}$ by taking into account both how the solution changes in time and how different our current update is from the optimizer at each time step. To do this, we set up a prediction-correction scheme, much like a Kalman filter strategy in estimation theory. In the first step, we will predict how the solution changes, and in the correction step we will do one step of gradient or Newton method towards the optimizer at that time instance. As mentioned in the Introduction, we call this strategy \emph{solution tracking}, to contrast it with standard \emph{running} algorithms that do not predict how the solution changes, but only adapt to it. 

\subsection{Prediction step}

To generate the prediction step, we reformulate the time-varying problem~\eqref{eq.problem} in terms of optimality conditions. Solving~\eqref{eq.problem} means to compute the solution of the following nonlinear system of equations
\begin{equation}
\nabla_{\x} f(\x^*(t); t) = \mathbf{0}, 
\end{equation}
for each $t$. For any other vector $\x$ (for example the approximate solution $\x_k$), we can write 
\begin{equation}\label{eq.isoerror}
\nabla_{\x} f(\x; t) = \r(t)
\end{equation}
where $\r(t)$ is some residual error. The aim of the prediction step is to keep this residual error as much fixed as possible while the optimization problem is changing. To say it in another way, we want to predict how to update $\x_k$ such that we stay close to the iso-residual manifold.  We can see how such trajectory evolves by perturbing it as
\begin{equation}
\nabla_{\x} f(\x; t) + \nabla_{\x\x} f(\x; t) \delta\x + \nabla_{t\x} f(\x; t) \delta t = \r(t),  
\end{equation}
and by using~\eqref{eq.isoerror} and by dividing it by $\delta t \neq 0$, we obtain the continuous dynamical system
\begin{equation}\label{eq.dyn}
\dot{\x} = - [\nabla_{\x\x} f(\x; t)]^{-1} \nabla_{t\x} f(\x; t). 
\end{equation}
By passing now in the discrete domain (where our algorithm will live), we sample the problem at sampling times $t_k$, for $k = 0,1,2,\dots$, and for the sake of simplicity we let this sampling be uniform, with sampling interval equal to $h$. We can integrate~\eqref{eq.dyn} by using a first-order forward Euler scheme as   
\begin{multline}\label{eq.up}
{\x}(t_{k+1}) = \x(t_{k}) - [\nabla_{\x\x} f(\x(t_k); t_k)]^{-1} \nabla_{t\x} f(\x(t_k); t_k) \, h \\ + \Delta,
\end{multline}
where $\Delta$ represents the discretization error. The discretization error can be upper bounded as follows. 

\begin{proposition}\label{prop.err}
Under Assumptions~\ref{as.0}, \ref{as.str}, and \ref{as.smooth}, the discretization error $\Delta$ of the Euler method~\eqref{eq.up} w.r.t. the real dynamics~\eqref{eq.dyn} is upper bounded by
$$
\Delta \leq \frac{h^2}{2}\left[\frac{C_0 C_2}{m^2} + \frac{C_3}{m}\right] = O(h^2).
$$
\end{proposition}
\vskip2mm

\begin{proof}
See Appendix~\ref{ap.prop}.
\end{proof}
\vskip2mm

Proposition~\ref{prop.err} says that under our assumptions we can use the Euler method. We will forget for the moment of the constant in the discretization error and live with its order in $h$ only. We can use the update rule~\eqref{eq.up} as the basics of our prediction step. Let ${\x}_{k+1|k}$ be the predicted decision variable vector; this will be computed as
\begin{equation}\label{eq:update}
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h.
\end{equation}


\subsection{Correction step}

The correction step can be devised by using, for example, a constant stepsize  projected gradient method based on the updated objective function at time $t_{k+1}$
\begin{equation}\label{eq.corr}
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \gamma \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})],
\end{equation}
for a choice of stepsize $\gamma > 0$, and where $P_{X}$ is the projection operator. Another way to design the correction step would be to use projected Newton's method; we will see how to perform that in Section~\ref{sec:newton}.  


{\color{green} [Here some words on the algorithm!]}


\subsection{Convergence analysis}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Centralized solution tracking (gradient-based)}
\label{alg.centr}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h
$$
\textbf{2:} Correction step:
$$
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \gamma \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})]
$$ 
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%

In Algorithm~\ref{alg.centr}, we summarize the devised centralized algorithm, whose convergence is encoded in the following theorem. 

\begin{theorem}\label{th.centr}
Let Assumption~\ref{as.0}, \ref{as.str}, and \ref{as.smooth} hold and let $\{\x_k\}$ be the sequence generated by Algorithm~\ref{alg.centr}. Define the rates $\rho$ and $\sigma$ as
%
\begin{equation}\label{thm:rho_sigma}
\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}, \quad \sigma = 1 + h(C_0 C_1/m^2 + C_2/m).
\end{equation}
%
\begin{enumerate}
\item If the sampling interval $h$ is chosen sufficiently small, then there exists a $\gamma>0$ for which 
\begin{equation*}
\rho \sigma < 1
\end{equation*}
and, in this case, convergence of $\{\x_k\}$ to $\x^*(t_k)$ is Q-linear up to a bounded error as,
\begin{equation}\label{result1}
\|{\x}_{k} - \x^*(t_{k})\| \leq (\rho \sigma)^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h^2).
\end{equation}
\item Irrespectively of the selection of $h$, if we pick $\gamma < m/L^2$, then convergence goes as   
\begin{equation}\label{result2}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h).
\end{equation}
\end{enumerate} 
\end{theorem}
%
\vskip2mm
\begin{myproof}

In order to prove Theorem~\ref{th.centr}, we start by bounding the error in the prediction step by terms that depend on the functional smoothness and the discretization error using Taylor expansions. Then we bound the tracking error of the gradient step using standard convergence properties of gradient descent on strongly convex functions. By substituting the error improvement achieved in the correction step into the prediction step, we establish the main result.

First, we establish that the criteria in which the bound stated in \eqref{result1} may be satisfied, i.e. that $\rho \sigma$ can be made strictly less than one, for a sufficiently small $h$. Note that, since $m>0$, there is always a $\gamma$ that makes $\rho < 1$ since $\gamma < m/L^2$. In particular, if we take $\gamma = m/ 2 L^2$, then $\rho$ is minimized and it is equal to 
%
\begin{equation}\label{rho}
\rho^* = \sqrt{ 1 - \frac{m^2}{4 L^2}}. 
\end{equation}
%
The coefficient $\sigma$ is a monotonically increasing function in $h$, and it is equal to $1$ when $h = 0$; by continuity of $\sigma$ in $h$, we can always find a small enough stepsize $h$, such that $\sigma < 1/\rho^*$, which means that we can find a stepsize $\gamma$ that yields $\rho \sigma <1$.

Now we turn to establishing the discrete-time sampling error bound stated in \eqref{result1} is achieved by the updates \eqref{eq:update}-\eqref{eq.corr}. For simplicity, we modify the notation to omit the arguments $\x_k$ and $t_k$ of the function $f$. In particular, define $\nabla_{\x\x}f = \nabla_{\x\x}f(\x_k; t_k)$, $\nabla_{t\x} f = \nabla_{t\x} f(\x_k; t_k)$, $\nabla_{\x\x}f^* = \nabla_{\x\x}f({\x}^*(t_{k}); t_k)$, and $\nabla_{t\x} f^* = \nabla_{t\x} f({\x}^*(t_{k}); t_{k})$. 

Begin by considering the update~\eqref{eq:update}, the prediction step, evaluated at a generic point $\x_k$ sampled at the current sample time $t_k$ and with associated optimizer $\x^*(t)$, which due to optimality will have null residual vector $\r(t) = \mathbf{0}$. Thus we may write
%
\begin{equation*}\left\{\begin{array}{rcl}
{\x}_{k+1|k} &=& \x_{k} - [\nabla_{\x\x}f]^{-1}\nabla_{t\x} f\,h\\
{\x}^*(t_{k+1}) &=& {\x}^*(t_{k}) - [\nabla_{\x\x}f^*]^{-1} \nabla_{t\x} f^*\,h + O(h^2).
\end{array}\right.
\end{equation*}
%
By subtracting one from the other and by considering the norm of the result, we obtain 
%
\begin{align}\label{eq.imp}
\|{\x}_{k+1|k}& -  \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\|  \\  & + \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h + O(h^2) .\nonumber 
\end{align}
%
Set the second term in the right-hand side of \eqref{eq.imp} as  $a= \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h$. We may rewrite $a$ by adding and subtracting the Newton step with the Hessian evaluated at the current optimal point,  $[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f$, to obtain
%
\begin{align}\label{eq.hessian_cross_term}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h,
\end{align}
%
We may bound the first and second-order derivative terms in the previous expression \eqref{eq.hessian_cross_term} by using Assumption~\ref{as.smooth} regarding the functional smoothness as well as the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} to write
%
\begin{equation}\label{eq.a}
a  \leq C_0 h \left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We now further bound the first term of the right-hand-side. To do that, we use the non-singularity of the Hessian to write 
%
\begin{multline}\label{eq.dummy10_midstep}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| = \\ \|[\nabla_{\x\x}f^*]^{-1}(\nabla_{\x\x}f - \nabla_{\x\x}f^*)[\nabla_{\x\x}f]^{-1} \|,
\end{multline} 
%
which by employing, once again, the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} we can bound as
\begin{equation}\label{eq.dummy10}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| \leq \frac{1}{m^2}\|\nabla_{\x\x}f - \nabla_{\x\x}f^* \|,
\end{equation} 
%
and therefore~\eqref{eq.a} can be written as
\begin{equation}\label{eq.amid}
a  \leq \frac{C_0}{m^2} h \left\|\nabla_{\x\x}f - \nabla_{\x\x}f^*\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We consider the Taylor expansion of the mixed second-order terms and the second-order terms in \eqref{eq.amid}, and apply the Mean Value Theorem with $\tilde{\x}$ as a point on the line between $\x_k$ and $\x^*(t_k)$ to obtain the following expressions,
%
\begin{subequations}\label{eq.dummy11}
\begin{multline}
\left\| \nabla_{\x\x} f- \nabla_{\x\x} f^*  \right\| \leq \left\|\nabla_{\x \x\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \\ \leq C_1 \|\x_k - \x^*(t_k)\|
\end{multline}
\begin{multline}
\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| \leq \left\|\nabla_{\x t\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \\ \leq C_2 \|\x_k - \x^*(t_k)\|
\end{multline}
\end{subequations}
%
The expressions in \eqref{eq.dummy11} may be substituted together into~\eqref{eq.amid} to yield
 %
\begin{align}
a  &\leq \frac{C_0 C_1 h}{m^2}\|\x_k - \x^*(t_k)\| + \frac{C_2 h}{m}\|\x_k - \x^*(t_k)\|.
\end{align}
%
Now we can use this bound for $a$ in~\eqref{eq.imp} to get
%
\begin{multline*}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \\ \Big[1 + h\left(\frac{C_0 C_1 h}{m^2} + \frac{C_2 h}{m}\right) \Big]\|{\x}_{k} - \x^*(t_{k})\| + O(h^2).
\end{multline*}
%
which, by the definition of $\sigma$ as stated in \eqref{thm:rho_sigma} in Theorem \ref{th.centr}, allows us to conclude
%
\begin{equation}\label{eq.fin1}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \sigma \|{\x}_{k} - \x^*(t_{k})\| + O(h^2).
\end{equation}
%
For the correction step [cf. \eqref{eq.corr}] , we may use the standard property of projected gradient descent for strongly convex functions. In particular, the gradient converges Q-linearly as
%
\begin{equation}\label{eq.fin2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \|{\x}_{k+1|k} - \x^*(t_{k+1})\|
\end{equation}
%
where $\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}$, see \cite{Nesterov2004} for further details.
%
%\subsection{Total algorithm}

We are ready to consider the combined error bound achieved by the prediction-correction scheme. By plugging the correction error \eqref{eq.fin2} into the prediction error \eqref{eq.fin1} we obtain
%
\begin{equation}\label{eq.fin_t_k}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \sigma \|{\x}_{k} - \x^*(t_{k})\| + \rho O(h^2).
\end{equation}
%
Now recursively apply the relationship \eqref{eq.fin_t_k} backwards in time to the initial time sample at $t_0$ to write
%
\begin{equation*}\label{eq.fin_t_0}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq (\rho \sigma)^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h^2),
\end{equation*}
%
which is the result \eqref{result1} in Theorem \ref{th.centr}.

To establish the result stated in \eqref{result2} of Theorem \ref{th.centr}, observe that in the worst case, we may upper bound the term $a$ in \eqref{eq.amid} by using the bounds in Assumption \ref{as.smooth} to obtain the right hand side of the following expression 
%
\begin{align}\label{eq.worst_case}
a  & \leq  \frac{C_0 h}{m^2}
 \|\nabla_{\x\x}f - \nabla_{\x\x}f^*\| 
 + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| \nonumber\\
 & \leq \frac{2 C_0 L h}{m^2} + \frac{2 C_0 h}{m} = O(h),
\end{align}
%
Remembering the definition of the nonnegative scalar term $a=\left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h $ and substituting the bound~\eqref{eq.worst_case} into \eqref{eq.imp}, we can write
%
\begin{equation}\label{eq.a_subst}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\| + O(h).
\end{equation}
%
This, together with the contraction property of the gradient step as stated in \eqref{eq.fin2} yields
%
\begin{equation}\label{eq.sampling_error2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho \|{\x}_{k} - \x^*(t_{k})\| + \rho O(h).
\end{equation}
%
If we iterate the expression \eqref{eq.sampling_error2} backwards in time to the initial point ${\x}_{0}$, we obtain
%
\begin{equation}\label{eq.rho_error_dependence}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h),
\end{equation}
%
which is~\eqref{result2}. With $\rho= \sqrt{1 + \gamma^2 L^2 - \gamma m}$ as defined in \eqref{thm:rho_sigma}, we only need to find a $\gamma$ that makes $\rho < 1$. Selecting any $\gamma$  satisfying $\gamma < m/L^2 $ concludes the proof.

\end{myproof}


\vskip2mm
\begin{corollary}\label{co.centr}
Under the same conditions of Theorem~\ref{th.centr},
\begin{enumerate}
\item If we pick $\gamma = m/2 L^2$, then the convergence bounded error is between $O(h)$ and $O(h^2)$. 
\item If we do not perform the prediction step in Algorithm~\ref{alg.centr} but only the correction step (i.e., we use Algorithm~\ref{alg.centr} as a running algorithm), then, if we pick $\gamma < m/L^2$, convergence goes as 
\begin{equation*}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^{k} \|{\x}_{0} - \x^*(t_{0})\| + \frac{\rho}{1-\rho} O(h).
\end{equation*}
\end{enumerate}
\end{corollary}
%
\vskip2mm
\begin{myproof}

Point 1) follows from the proof of Theorem~\ref{th.centr}. In fact, if we select $\gamma = m/2 L^2$ then we minimize $\rho$ (as stated in~\eqref{rho}). Therefore, with this selection of $\gamma$, two cases are possible. 

The first case is that $h$ is small enough, such that $\rho \sigma < 1$. Here, we can use the first part of Theorem~\ref{th.centr} and, in particular, Equation~\eqref{result1}, which brings a bounded error of size $O(h^2)$. 

The second case is that $h$ is not small enough, such that $\rho \sigma \geq 1$. Here, we can use the second part of Theorem~\ref{th.centr}, i.e., Equation~\eqref{result2}, to bound the asymptotical error to $O(h)$. 

By putting together the two cases, the claim of Point 1) follows. 

Point 2) also follows directly from the proof of Theorem~\ref{th.centr}. Suppose that we execute the correction step \eqref{eq.corr} without the prediction step \eqref{eq:update}. Such an update would be equivalent to performing the updates \eqref{eq:update}-\eqref{eq.corr} with the prediction step evaluated at $\nabla_{t\x} f = {\bf{0}}$. Substituting this case into \eqref{eq.imp} yields
\begin{align*}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| &\leq \|{\x}_{k} - \x^*(t_{k})\| \\
 & \qquad + \left\|[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h 
	+ O(h^2) \\ 
	&\leq \|{\x}_{k} - \x^*(t_{k})\| + \frac{C_0 h}{m} + O(h^2) \\
	 & \leq \|{\x}_{k} - \x^*(t_{k})\| + O(h),
\end{align*}
%
where we have bounded the magnitude of the Hessian and the derivative mixed first order derivative terms using Assumptions \ref{as.str}-\ref{as.smooth}, respectively. From here, the analysis proceeds exactly as from \eqref{eq.a_subst} to the conclusion of 2) in Theorem~\ref{th.centr}, yielding \eqref{eq.rho_error_dependence}, which concludes the proof. 

\end{myproof}

\vskip2mm
Theorem~\ref{th.centr} says that our tracking algorithm generates a converging sequence of approximate solutions and the error bound depends (at worst) linearly on the sampling interval. Convergence is quite fast (in fact Q-linear), as one would expect in strongly convex problems. Corollary~\ref{co.centr} confirms our intuition that performing the prediction step improves upon state-of-the-art running algorithms (passing from an error bound of $O(h)$ to $O(h^2)$ if $h$ is chosen small enough). 


\begin{remark}\label{rem.k}
We can readily extend the results on this section and the following one when the constant $C_0, C_1, C_2, m, L$ are constant in the decision variable $\x$ but not uniformly in time. In order to do that, we have to substitute these constants by other ones, depending on the sampled time instance $t_k$ as $C_{0,k}, C_{1,k}, C_{2,k}, m_k, L_k$. With this substitution, all the results hold true (with minor modifications) and in particular the stepsize $\gamma$ can be chosen to vary from $k$ to $k+1$. 
\end{remark}


\section{Newton correction}\label{sec:newton}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Centralized solution tracking (Newton-based)}
\label{alg.newton}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h.
$$
\textbf{2:} Correction step:
\begin{multline*}
{\x}_{k+1} = P_{X}[\x_{k+1|k} - \\ [\nabla_{\x\x} f(\x_{k+1|k}; t_{k+1})]^{-1} \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})]
\end{multline*}
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%
In this section, we explore the possibility of using a Newton's step for the correction step in Algorithm~\ref{alg.centr}. We want to see if substituting~\eqref{eq.corr} with 
\begin{multline}
{\x}_{k+1} = \x_{k+1|k} - [\nabla_{\x\x} f(\x_{k+1|k}; t_{k+1})]^{-1}\times\\ \nabla_{t\x} f(\x_{k+1|k}; t_{k+1})
\end{multline}
yields a further decrease in the asymptotic error from $O(h^2)$ to something smaller than that. Intuitionally that should be the case, since Newton's method has local quadratic convergence, so we expect to reduce $O(h^2)$ to a $O(h^4)$ error. In this section, we will prove that this is not in general the case, which undermines the usefulness of a Newton's correction step in time-varying problems. 


In particular, we analyze the local convergence of Algorithm~\ref{alg.newton}. 

\begin{theorem}\label{th.newton}
Let Assumptions~\ref{as.0}, \ref{as.str}, and \ref{as.smooth} hold true. Suppose the initial guess $\x_0$ is picked close enough to the initial optimizer, i.e., the norm $\|\x_0 - \x^*(t_0)\| \leq \alpha h^2 /2$, with $\alpha h^2 /2 \ll 1$. Define the parameter $\alpha' = [C_0 C_2/ m^2 + C_3/m]$, so that the Euler discretization error $\Delta$ in Proposition~\ref{prop.err} has the worst case value of $\Delta = \alpha' h^2/2$. In addition, suppose that this worst case value is small enough, i.e., $\alpha' h^2/2 \ll 1$. With this in place, for the sequence $\{\x_k\}$ generated by Algorithm~\ref{alg.newton} we have for all $k>1$
\begin{enumerate}
\item if $C_1/2 m \leq 2\alpha/[(\alpha + \alpha')^2\, h^2]$, then 
$$
\|\x_k - \x^*(t_k)\| \leq O(h^2),
$$
\item if, in addition, $C_1/2 m \leq 1$, then 
$$
\|\x_k - \x^*(t_k)\| \leq O(h^4).
$$
\end{enumerate}
\end{theorem}
\vskip2mm

\begin{proof}
See Appendix~\ref{ap.newton}. 
\end{proof}
\vskip2mm

Theorem~\ref{th.newton} says that, in general, if we select $h$ small enough, we can track the optimizer $\x^*(t_k)$ at worst with a $O(h^2)$ error bound. This is very similar to the result we had for the gradient-based tracking algorithm. In special cases, when $C_1/2m \leq 1$, then the quadratic convergence of the Newton's method appears and we track the optimizer at worst with a error bound of $O(h^4)$. A special case of the second situation are quadratic cost functions, for which $C_1 = 0$, and we have perfect convergence. 

%We will see in the simulation results in Section~\ref{sec:num} that, in practice, since both $C_1$ and $m$ vary in time, Algorithm~\ref{alg.newton} generates a sequence that oscillates between a $O(h^2)$ error level and a $O(h^4)$ one, thereby making a Newton's correction step less useful, beyond limited special cases.   


\section{Approximate time derivative}\label{sec:app}

In several situations, we are not provided with the knowledge of how the function changes in time. 

\textcolor{red}{In which situations would one expect to need to do such an approximation? Is there a connection to stochastic control in discrete time?}

In these situations, to still be able to use our algorithms, we need to estimate the term $\nabla_{t\x} f(\x; t)$ is some ways. Let $\tilde{\nabla}_{t\x}{f}_k$ be an approximate version of $\nabla_{t\x}f(\x_k; t_k)$. Examples of such approximate version are the following. 

%We notice that most of the analysis in Theorem~\ref{th.centr} and \ref{th.net} carries trough unchanged. The only addition in the proofs is that we need to consider the extra source of error
%\begin{equation}\label{extraerr}
%\frac{h}{m}\|\tilde{\nabla}_{t\x}{f}_k -  \nabla_{t\x}f(\x_k; t_k)\| 
%\end{equation}
%which can be easily bounded once $\tilde{\nabla}_{t\x}{f}_k$ is available. Examples are the following.

\vskip2mm
\noindent\textbf{First-order backward derivative.} We can approximate the derivative as 
\begin{equation}\label{fobd}
\tilde{\nabla}_{t\x}{f}_k = \frac{1}{h} (\nabla_{\x}f(\x_k; t_k) - \nabla_{\x}f(\x_{k-1}; t_{k-1})),
\end{equation}
which has an approximation error of $O(h)$. %This combined with the $h$ factor in~\eqref{extraerr} brings the additional error to an $O(h^2)$ level.

\vskip2mm
\noindent\textbf{Higher-order backward derivative.} We can approximate the derivative recursively as
\begin{multline*}
\tilde{\nabla}_{t\x}{f}_k = \frac{1}{h}\left(a \nabla_{\x}f(\x_k; t_k) + b \nabla_{\x}f(\x_{k-1}; t_{k-1})\right. \\ \left.+ c \nabla_{\x}f(\x_{k-2}; t_{k-2}) + d\nabla_{\x}f(\x_{k-3}; t_{k-3})\right) - \beta \tilde{\nabla}_{t\x}{f}_{k-1},
\end{multline*}
which, if we specify the coefficient $(a,b,c,d,\beta)$ properly, leads to an approximation error of $O(h^2)$, $O(h^3)$, or $O(h^4)$~\cite{Lee1992}. %and therefore yields an error of at least one order of magnitude lower than the existing error bound. 

\vskip2mm
In the next corollary, we quantify the additional error of approximating the time derivative in our prediction-correction Algorithm~\ref{alg.centr}. We further show that this error goes as $O(h^2)$ for a simple first-order backward derivative, thereby stating that estimating the time derivative is not detrimental for our scheme. 

\begin{corollary}\label{co.approx}
Under the same conditions of Theorem~\ref{th.centr}, if we approximate the time derivative $\nabla_{t\x}f(\x_k; t_k)$ by using a first-order backward derivative as in~\eqref{fobd}, the asymptotic error bound of Algorithm~\ref{alg.centr} is not worse than the one of Theorem~\ref{th.centr}.  
\end{corollary}
%
\vskip2mm
\begin{myproof}

By Taylor expansion, one can see that
\begin{equation}\label{appder_oh}
\|\tilde{\nabla}_{t\x}{f}_k  - {\nabla}_{t\x}{f}(\x_k; t_k)\| = O(h),  
\end{equation}
also proving the claimed $O(h)$ error bound of the first-order backward derivative. In fact, one Taylor expands
\begin{equation}
{\nabla}_{\x}{f}(\x_{k-1}; t_{k-1}) = {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h + O(h^2),
\end{equation} 
and by solving for ${\nabla}_{t\x}{f}(\x_k; t_k)$, 
\begin{equation}
{\nabla}_{t\x}{f}(\x_k; t_k) = \frac{1}{h} ( {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h + O(h^2)).
\end{equation}
By substituting this result and the definition~\eqref{fobd} into~\eqref{appder_oh}, the $O(h)$ error bound is proven. 

Consider now the approximate prediction step, 
\begin{equation}
\x_{k+1|k} = \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h,
\end{equation}
which by adding and subtracting the exact prediction direction becomes, 
\begin{align}
\x_{k+1|k} &= \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h + \nonumber \\ &\quad 
+[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h  \nonumber \\ &\quad - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h.
\end{align}
By following the same steps as in Theorem~\ref{th.centr}, the term $a$ in Equation~\eqref{eq.hessian_cross_term} can be written with an extra error term as, 
\begin{align}\label{eq.hessian_cross_term_2}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h \nonumber \\ &\quad + \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h.
\end{align}
%
The extra error term w.r.t. Equation~\eqref{eq.hessian_cross_term} can be further bounded by using~\eqref{appder_oh} and the smoothness Assumption~\ref{as.smooth} (with the strong convexity constrant $m$)
\begin{multline}
 \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h \leq \\
 \|[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1}\| \| {\nabla}_{t\x}{f}(\x_k; t_k)  - \tilde{\nabla}_{t\x}{f}_k \| \, h \leq \\
 \frac{1}{m} O(h) \, h = O(h^2).
\end{multline}
This means that the extra error is of size $O(h^2)$ so it will not increase the $O(h^2)$ error bound already proven in Theorem~\ref{th.centr}.

\end{myproof}

Corollary~\ref{co.approx} says that we can approximate the time derivative simply by a first-order scheme. Better approximation will not decrease the functional dependence of the error in $h$, but may decrease the its magnitude. In the simulation results we show that

{\color{green} [Finish.]}  

\section{Prediction-Correction$(s)$ algorithms}

%
%----------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{Prediction-Correction$(s)$ (gradient-based)}
\label{alg.pcs}
\footnotesize
%\begin{algorithmic}[1]
Pick an initial guess $\x_0$; for all $k\geq 0$ \\
\textbf{Input:} the previous approximate solution $\x_k$\\
\color{white}aa\color{black}\vrule \color{white}aa\color{black}\begin{minipage}{0.45\textwidth}
\vskip1mm
\textbf{1:} Prediction step: 
$$
{\x}_{k+1|k} = \x_k - [\nabla_{\x\x} f(\x_k; t_k)]^{-1} \nabla_{t\x} f(\x_k; t_k) \, h
$$
\textbf{2:} Correction step: \\
\hspace*{4mm} \textbf{Set} $\x_{k+1/s|k} = \x_{k+1|k}$\\
\hspace*{4mm} \textbf{For} $\tau=1$ to $s$ \textbf{do}
$$
{\x}_{k+\tau/s} = P_{X}[\x_{k+\tau/s|k} - \gamma \nabla_{t\x} f(\x_{k+\tau/s|k}; t_{k+1})]
$$ 
\hspace*{4mm} \textbf{End}
\end{minipage}\\ \vskip1mm
\textbf{Output:} the new approximate solution $\x_{k+1}$
%\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------
%


If we have enough computational power, we could always think to perform several correction steps (either of a gradient method or of a Newton's scheme), to further reduce the tracking asymptotical error. We call these algorithms Prediction-Correction$(s)$ algorithms (and they are parametrized over the number $s$ of correction steps. An example of such algorithm for gradient descent is given in Algorithm~\ref{alg.pcs}.

Convergence of such schemes can be proven in a similar fashion as in Theorem~\ref{th.centr}. As a bonus, in these schemes, the bigger $s$ is the larger $h$ can be chosen. This result as well as the convergence is encoded as follows. 

\begin{corollary}\label{co.pcs}
Under the same conditions of Theorem~\ref{th.centr}, Algorithm~\ref{alg.pcs} generates a sequence $\{\x_k\}$ that converges to $\x^*(t_k)$ asymptotically, with an error bound of 
$$
\lim_{k\to\infty} \|\x(t_k) - \x^*(t_k)\| = \frac{\rho^s}{1-\rho^s} O(h^2), \textrm{ if } \rho^s \sigma < 1, 
$$
and
$$
\lim_{k\to\infty} \|\x(t_k) - \x^*(t_k)\| = \frac{\rho^s}{1-\rho^s} O(h), \textrm{ if } \rho^s \sigma \geq 1, \rho < 1.
$$
In addition, if $s$ is selected as 
$$
s \geq \left\lceil \frac{p \log h}{\log(\rho(1 + h^p))}\right\rceil,
$$
then the asymptotical error is multiplied by a term $O(h^p)$.
\end{corollary}
%
\vskip2mm
\begin{myproof}

The proof is rather immediate and follows from the proof of Theorem~\ref{th.centr}. In particular, the only difference is in the correction step, which is performed $s$ times. Therefore, we can modify Equation~\eqref{eq.fin_t_k} as
$$
\|\x_{k+1} - \x^*(t_{k+1})\| \leq \rho^s \sigma \|\x_{k} - \x^*(t_{k})\| + \rho^s O(h^2),
$$
or Equation~\eqref{eq.sampling_error2} as 
$$
\|\x_{k+1} - \x^*(t_{k+1})\| \leq \rho^s \|\x_{k} - \x^*(t_{k})\| + \rho^s O(h),
$$
and the rest follows almost verbatim. The last result on the numbers of correction steps $s$ to obtain a certain error level, can be obtained directly by solving the equation
$$
\frac{\rho^s}{1-\rho^s} = h^p,
$$ 
for $s$. 

\end{myproof} 
















%\section{Approximate Hessian inverse}\label{sec:hess}





==> Proofs_1.tex <==

% !TEX root = TimeVarying_part1.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newpage
\section{Proof of Proposition~\ref{prop.err}}\label{ap.prop}

For the forward Euler method applied to the nonlinear dynamical system
%%%
\begin{equation}\label{proof_100}
\dot{x} = {\mathcal{F}}(x,t),
\end{equation}
%%%
the local discretization error is bounded by~\cite[Chapter~11]{Quarteroni2000} $h^2/2\, \|\mathrm{d}\mathcal{F}(x,t)/\mathrm{d}t\|$. We can extend this result, by considering that the forward Euler method is based on a truncated Taylor series expansion. Let us analyze the forward Euler method applied to the vector-valued nonlinear dynamical system
%%%
\begin{equation}\label{proof_110}
\dot{\x} = {\mathbold{F}}(\x,t).
\end{equation}
%%%
If we apply the forward Euler method to the relation in \eqref{proof_110}, starting at a certain point $\x(t_k)$, we obtain 
%%%
\begin{equation}\label{proof_120}
\x_{k+1} = \x(t_k)+ {\mathbold{F}}(\x(t_k),t_k)\, h. 
\end{equation}
%%%
Subtracting $\x(t_{k+1})$ from the both sides of the equality in \eqref{proof_120} and computing the norm of the resulted relation implies that
%%%
\begin{equation}\label{proof_130} 
\|\x_{k+1} - \x(t_{k+1})\| =  \left\|{\mathbold{F}}(\x(t_k),t_k)\, h  -\int_{t_k}^{t_{k+1}} \!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau \right\|.
\end{equation}
%%%%%
Notice that \eqref{proof_130} is resulted by considering the relation $\x(t_{k+1}) = \x(t_{k}) +\int_{t_k}^{t_{k+1}} {\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau$. Observe that according to the Mean Value theorem there exits a $\hat{\tau} \in [t_k, t_{k+1}]$ that satisfies 
%%%
\begin{equation}\label{proof_140} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau = \int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(t_k),t_k) + \nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,h \, \textrm{d} \tau.
\end{equation}
%%%%%
Notice that the term ${\mathbold{F}}(\x(t_k),t_k)$ does not depend on the integral variable $\tau$. Considering this observation and observing the definition $h:=t_{k+1}-t_k$, we can simplify the first part of the integral in the right hand side of \eqref{proof_140} as 
%
\begin{equation}\label{proof_145} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(t_k),t_k)  \textrm{d} \tau= {\mathbold{F}}(\x(t_k),t_k) h \; .
\end{equation}
%
 Since $\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau})$ is also not a function of variable $\tau$,   by applying the same argument we can simplify the second part of the integral in the right hand side of \eqref{proof_140} as
 %
 \begin{equation}\label{proof_147} 
  \int_{t_k}^{t_{k+1}}\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,h \, \textrm{d} \tau=\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,(h^2)/2 \;.
  \end{equation}
   Therefore, we can rewrite \eqref{proof_140} as 
%%%
\begin{equation}\label{proof_150} 
\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau = {\mathbold{F}}(\x(t_k),t_k)\ \!h + \nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau}) \,\frac{h^2}{2}.
\end{equation}
%%%%%
By substituting the integral $\int_{t_k}^{t_{k+1}} \!\!\!{\mathbold{F}}(\x(\tau),\tau)\, \textrm{d} \tau$ in \eqref{proof_130} by the simplification in \eqref{proof_150} and considering the definition of the discretization error vector $\mathbold{\Delta}:=\x_{k+1} - \x(t_{k+1})$ we can rewrite \eqref{proof_130} as
%%%
\begin{equation}\label{proof_160} 
\|\mathbold{\Delta} \|=  \frac{h^2}{2} \|\nabla_{t}{\mathbold{F}}(\x(\hat{\tau}),\hat{\tau})\|.
\end{equation}
%%%%%
Observing the continuous dynamical system in \eqref{eq.dyn} we know that ${\mathbold{F}}(\x,t)$ is given by
%%%
\begin{equation}\label{proof_170} 
{\mathbold{F}}(\x,t) = -[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t).
\end{equation}
%%%%%
We proceed to find an upper bound for the right hand side of \eqref{proof_160}. Note that based on the definition in \eqref{proof_170} we can write 
%%%
\begin{align}\label{proof_180} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|= \left\|\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]\right\|
\end{align}
%%%%%
Notice that by applying the chain rule we can simplify the derivative $\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]$ as
%%%
\begin{align}\label{proof_190} 
&\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]=\\
&\qquad\qquad\qquad[\nabla_{\x\x}f(\x; t)]^{-2} \nabla_{t \x\x}f(\x; t) \nabla_{t\x}f(\x; t)\nonumber\\
&
\qquad\qquad\qquad+ [\nabla_{\x\x}f(\x; t)]^{-1}\nabla_{tt\x}f(\x; t)\nonumber.
\end{align}
%%%%%
Compute the norm of both sides of \eqref{proof_190}. Substitute the norm $\|\nabla_{t}\left[[\nabla_{\x\x}f(\x;t)]^{-1} \nabla_{t\x}f(\x;t)\right]\|$ by $\|\nabla_{t}{\mathbold{F}}(\x,t) \|$ as shown in \eqref{proof_180}. Further apply the triangle inequality to the right hand side of the resulted expression to obtain 
%%%
\begin{align}\label{proof_200} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|&\leq\left\|[\nabla_{\x\x}f(\x; t)]^{-2} \nabla_{t \x\x}f(\x; t) \nabla_{t\x}f(\x; t)\right\|\nonumber\\
&
\quad+ \left\|[\nabla_{\x\x}f(\x; t)]^{-1}\nabla_{tt\x}f(\x; t)\right\|.
\end{align}
%%%%%
Observe the fact that $\nabla_{t \x\x}f(\x; t) = \nabla_{\x t\x}f(\x; t)$. We use the Cauchy-Schwartz inequality and the bounds in Assumptions \ref{as.str} and  \ref{as.smooth} to update the upper bound in \eqref{proof_200} as
%%%
\begin{align}\label{proof_210} 
\|\nabla_{t}{\mathbold{F}}(\x,t) \|  \leq \frac{C_0 C_2}{m^2} + \frac{C_3}{m}
\end{align}
%%%%%
Combining the relation in \eqref{proof_160} and the upper bound in \eqref{proof_210} follows the claim in \eqref{prop_claim_err_bound}.
%%
\qed 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem \ref{th.GTT_convg}}\label{app.GTT_convg}


In order to prove Theorem \ref{th.GTT_convg}, we start by bounding the error in the prediction step by the terms that depend on the functional smoothness and the discretization error using Taylor expansions. Then we bound the tracking error of the gradient step using standard convergence properties of gradient descent on strongly convex functions. By substituting the error improvement achieved in the correction step into the prediction step, we establish the main result.

First, we establish that the criteria in which the bound stated in \eqref{result1} may be satisfied, i.e. that $\rho \sigma$ can be made strictly less than 1, for a sufficiently small $h$. Note that, since $m>0$, there is always a $\gamma$ that makes $\rho < 1$ since $\gamma < m/L^2$. In particular, if we take $\gamma = m/ 2 L^2$, then $\rho$ is minimized and it is equal to 
%
\begin{equation}\label{rho}
\rho^* = \sqrt{ 1 - \frac{m^2}{4 L^2}}. 
\end{equation}
%
The coefficient $\sigma$ is a monotonically increasing function in $h$, and it is equal to $1$ when $h = 0$; by continuity of $\sigma$ in $h$, we can always find a small enough stepsize $h$, such that $\sigma < 1/\rho^*$, which means that we can find a stepsize $\gamma$ that yields $\rho \sigma <1$.

Now we turn to establishing the discrete-time sampling error bound stated in \eqref{result1} is achieved by the updates \eqref{GTT_prediction}-\eqref{GTT_correction}. For simplicity, we modify the notation to omit the arguments $\x_k$ and $t_k$ of the function $f$. In particular, define 
%
\begin{align}\label{eq:thm1_defs}
&\nabla_{\x\x}f = \nabla_{\x\x}f(\x_k; t_k)\; , &&\nabla_{t\x} f = \nabla_{t\x} f(\x_k; t_k)\;,\nonumber \\ 
&\nabla_{\x\x}f^* = \nabla_{\x\x}f({\x}^*(t_{k}); t_k)\;,  && \nabla_{t\x} f^* = \nabla_{t\x} f({\x}^*(t_{k}); t_{k}) \; . \nonumber
\end{align}
%
Begin by considering the update~\eqref{GTT_prediction}, the prediction step, evaluated at a generic point $\x_k$ sampled at the current sample time $t_k$ and with associated optimizer $\x^*(t)$, which due to optimality will have null residual vector $\r(t) = \mathbf{0}$. Thus we may write
%
\begin{equation}\label{eq:null_residual}
\left\{\begin{array}{rcl}
{\x}_{k+1|k} &=& \x_{k} - [\nabla_{\x\x}f]^{-1}\nabla_{t\x} f\,h\\
{\x}^*(t_{k+1}) &=& {\x}^*(t_{k}) - [\nabla_{\x\x}f^*]^{-1} \nabla_{t\x} f^*\,h + \Delta.
\end{array}\right.
\end{equation}
%
By subtracting one from the other and by considering the norm of the result, we obtain 
%
\begin{align}\label{eq.imp}
\|{\x}_{k+1|k}& -  \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\|  \\  & + \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h + \|\mathbold{\Delta}\| .\nonumber 
\end{align}
%
Define $a$ as the second term in the right-hand side of \eqref{eq.imp}, as  $a= \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h$. We may rewrite $a$ by adding and subtracting the Newton step with the Hessian evaluated at the current optimal point,  $[\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f$, to obtain
%
\begin{align}\label{eq.hessian_cross_term}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\ &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h,
\end{align}
%
We may bound the first and second-order derivative terms in the previous expression \eqref{eq.hessian_cross_term} by using Assumption~\ref{as.smooth} regarding the functional smoothness as well as the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} to write
%
\begin{equation}\label{eq.a}
a  \leq C_0 h \left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We now further bound the first term of the right-hand-side. To do that, we use the non-singularity of the Hessian to write 
%
\begin{multline}\label{eq.dummy10_midstep}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| = \\ \|[\nabla_{\x\x}f^*]^{-1}(\nabla_{\x\x}f - \nabla_{\x\x}f^*)[\nabla_{\x\x}f]^{-1} \|,
\end{multline} 
%
which by employing, once again, the strong convexity constant $m$ of the Hessian in Assumption \ref{as.str} we can bound as
\begin{equation}\label{eq.dummy10}
\left\|[\nabla_{\x\x}f]^{-1} - [\nabla_{\x\x}f^*]^{-1}\right\| \leq \frac{1}{m^2}\|\nabla_{\x\x}f - \nabla_{\x\x}f^* \|,
\end{equation} 
%
and therefore~\eqref{eq.a} can be written as
\begin{equation}\label{eq.amid}
a  \leq \frac{C_0}{m^2} h \left\|\nabla_{\x\x}f - \nabla_{\x\x}f^*\right\| + \frac{h}{m}\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\|.
\end{equation}
%
We consider the Taylor expansion of the mixed second-order terms and the second-order terms in \eqref{eq.amid}, and apply the Mean Value Theorem with $\tilde{\x}$ as a point on the line between $\x_k$ and $\x^*(t_k)$ to obtain the following expressions,
%
%\begin{subequations}
\begin{align} \label{eq.dummy11}
\left\| \nabla_{\x\x} f- \nabla_{\x\x} f^*  \right\| &
\leq \left\|\nabla_{\x \x\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \nonumber\\ 
&\leq C_1 \|\x_k - \x^*(t_k)\| \\
%\end{multline}
%\begin{multline}
\left\| \nabla_{t\x} f- \nabla_{t\x} f^*  \right\| &
\leq \left\|\nabla_{\x t\x} f(\tilde{\x}; t_k)\right\| \|\x_k - \x^*(t_k)\| \nonumber \\
& \leq C_2 \|\x_k - \x^*(t_k)\| \label{eq.dummy111}
\end{align}
%\end{subequations}
%
The expressions in \eqref{eq.dummy11} - \eqref{eq.dummy111} may be substituted together into~\eqref{eq.amid} to yield
 %
\begin{align}
a  &\leq \frac{C_0 C_1 h}{m^2}\|\x_k - \x^*(t_k)\| + \frac{C_2 h}{m}\|\x_k - \x^*(t_k)\|.
\end{align}
%
Now we can use this bound for $a$ in~\eqref{eq.imp} to get
%
\begin{align}\label{some_bound}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq&  \Big[1 + h\left(\frac{C_0 C_1 h}{m^2} + \frac{C_2 h}{m}\right) \Big] \times \nonumber \\
& \quad \|{\x}_{k} - \x^*(t_{k})\| + \|\mathbold{\Delta}\|.
\end{align}
%
By considering the definition of $\sigma$ in \eqref{thm:rho_sigma} and substituting the discretization error norm $\|\mathbold{\Delta}\|$ by its upper bound in \eqref{prop_claim_err_bound}, we obtain that
%
\begin{equation}\label{eq.fin1}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \sigma \|{\x}_{k} - \x^*(t_{k})\| + \frac{h^2}{2}\left[\frac{C_0 C_2}{m^2} + \frac{C_3}{m}\right] .
\end{equation}
%
For the correction step [cf. \eqref{GTT_correction}] , we may use the standard property of projected gradient descent for strongly convex functions. In particular, the gradient converges Q-linearly as
%
\begin{equation}\label{eq.fin2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\| \leq \rho \|{\hat{\x}}_{k+1}^{s} - \x^*(t_{k+1})\| .
\end{equation}
%
where $\rho = \sqrt{1 + \gamma^2 L^2 - \gamma m}$. To see this, it is sufficient to write the projected gradient step as 
\begin{multline}\label{eq.explanation1}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 = \\  \|P_X[{\hat{\x}}_{k+1}^{s} -\gamma \nabla_{\x} f(\hat{\x}_{k+1}^s; t_{k+1})] - \x^*(t_{k+1})\|^2 .
\end{multline}
Since $\x^*(t_{k+1}) = P_X[\x^*(t_{k+1})-\gamma\nabla_{\x} f(\x^*(t_{k+1}), t_{k+1})]$ for optimality, and since the projection is nonexpansive, we obtain 
\begin{multline}\label{eq.explanation2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 \leq  \|{\hat{\x}}_{k+1}^{s}  - \x^*(t_{k+1}) \\- \gamma (\nabla_{\x} f(\hat{\x}_{k+1}^s; t_{k+1}) - \nabla_{\x} f(\x^*(t_{k+1}), t_{k+1}) )\|^2 .
\end{multline}
By expanding the right-hand side and by the strong convexity and functional smoothness assumptions (Assumptions~\ref{as.str} and \ref{as.smooth}), we can write
\begin{equation}\label{eq.explanation2}
\|{\hat{\x}}_{k+1}^{s+1} - \x^*(t_{k+1})\|^2 \! \leq \! (1+\gamma^2L^2-\gamma m)\|{\hat{\x}}_{k+1}^{s} - \x^*(t_{k+1})\|^2 .
\end{equation}
which is~\eqref{eq.fin2}. 
%see \cite{Nesterov2004} for further details. 
%
%
%
Observe that the sequence ${\hat{\x}}_{k+1}^{s}$ is initialized by the predicted variable $\x_{k+1|k}$ and the corrected variable $\x_{k+1}$ is equal to $ {\hat{\x}}_{k+1}^{\tau}$. Considering these observation and the relation in \eqref{eq.fin2} between two consecutive iterates of the sequence ${\hat{\x}}_{k+1}^{s}$ we can write 
%
\begin{equation}\label{eq.fin222}
\|{{\x}}_{k+1}- \x^*(t_{k+1})\| \leq \rho^\tau \|\x_{k+1|k} - \x^*(t_{k+1})\| .
\end{equation}
%
We are ready to consider the combined error bound achieved by the prediction-correction scheme. By plugging the correction error in \eqref{eq.fin222} into the prediction error in \eqref{eq.fin1} we obtain
%
\begin{equation}\label{eq.fin_t_k}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^\tau \sigma \|{\x}_{k} - \x^*(t_{k})\| +  \rho^\tau \Gamma,
\end{equation}
%
where $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$ is defined to simplify the notation. Notice that the relation between $\|{\x}_{k+1} - \x^*(t_{k+1})\|$ and $\|{\x}_{k} - \x^*(t_{k})\| $ in \eqref{eq.fin_t_k} is also holds true for $\|{\x}_{k} - \x^*(t_{k})\| $ and $\|{\x}_{k-1} - \x^*(t_{k-1})\| $. I.e., 
%
\begin{equation}\label{eq.fin_t_k_1}
\|{\x}_{k} - \x^*(t_{k})\| \leq \rho^\tau \sigma \|{\x}_{k-1} - \x^*(t_{k-1})\| +  \rho^\tau \Gamma.
\end{equation}
%
Substituting the upper bound in \eqref{eq.fin_t_k_1} for $\|{\x}_{k} - \x^*(t_{k})\|$ into \eqref{eq.fin_t_k} implies an upper bound for $\|{\x}_{k+1} - \x^*(t_{k+1})\| $ in terms of the norm difference for time $k-1$ as
%
\begin{align}\label{eq.fin_t_k_new}
\|{\x}_{k+1} - \x^*(t_{k+1})\| &\leq (\rho^\tau \sigma)^2 \|{\x}_{k-1} - \x^*(t_{k-1})\|
\nonumber \\
& \qquad +\rho^\tau \Gamma(\rho^\tau \sigma+1) .
\end{align}
%
Now recursively apply the relationship \eqref{eq.fin_t_k} backwards in time to the initial time sample and use the same argument form \eqref{eq.fin_t_k} to \eqref{eq.fin_t_k_new} to write 
%
\begin{equation}\label{eq.fin_t_00}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq (\rho^\tau \sigma)^{k+1} \|{\x}_{0} - \x^*(t_{0})\| + \rho^\tau \Gamma \sum_{i=0}^k (\rho^\tau\sigma)^i.
\end{equation}
%
Substituting $k+1$ by $k$ and simplifying the sum in \eqref{eq.fin_t_00} leads to
%
\begin{equation}\label{eq.fin_t_0000}
\|{\x}_{k} - \x^*(t_{k})\| \leq (\rho^\tau \sigma)^{k} \|{\x}_{0} - \x^*(t_{0})\| + \rho^\tau \Gamma \left[ \frac{1-(\rho^\tau\sigma)^k}{1-\rho^\tau\sigma}\right].
\end{equation}
%
Considering the result in \eqref{eq.fin_t_0000} and the definition for the constant $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$, the result in \eqref{result1} follows.

To establish the result stated in \eqref{result2}, observe that in the worst case, we may upper bound the term $a$ in \eqref{eq.amid} by using the bounds in Assumption \ref{as.smooth} to obtain the right hand side of the following expression 
%
\begin{align}\label{eq.worst_case}
a  
 & \leq \frac{2 C_0 L h}{m^2} + \frac{2 C_0 h}{m}.
\end{align}
%
Remembering the definition of the nonnegative scalar term $a:=\left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\| h $ and substituting the bound~\eqref{eq.worst_case} into \eqref{eq.imp}, we can write
%
\begin{multline}\label{eq.a_subst}
\|{\x}_{k+1|k} - \x^*(t_{k+1})\| \leq \|{\x}_{k} - \x^*(t_{k})\| \\ + h\left(\frac{2 C_0 L }{m^2} + \frac{2 C_0 }{m}\right) +  \|\mathbold{\Delta}\|.
\end{multline}
%
To simplify the notation we define a new constant $\Gamma_2:= h\left(({2 C_0 L }/{m^2} )+ ({2 C_0 }/{m})\right)$. Considering this definition and observing the  the relation in \eqref{eq.fin222} we can write 
%
\begin{equation}\label{eq.sampling_error2}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^\tau \|{\x}_{k} - \x^*(t_{k})\| + \rho^\tau (\Gamma_2 + \Gamma).
\end{equation}
%
%
Now recursively apply the relationship \eqref{eq.sampling_error2} backwards in time to the initial time sample and use the same argument form \eqref{eq.fin_t_k} to \eqref{eq.fin_t_0000} to write 
%
\begin{multline}\label{eq.rho_error_dependence}
\|{\x}_{k+1} - \x^*(t_{k+1})\| \leq \rho^{\tau(k+1)} \|{\x}_{0} - \x^*(t_{0})\| \\ +  \rho^\tau (\Gamma_2 + \Gamma) \left[ \frac{1-\rho^{\tau (k+1)}}{1-\rho^\tau}\right].
\end{multline}
%
Note that relation \eqref{eq.rho_error_dependence} shows an upper bound for $\|{\x}_{k+1} - \x^*(t_{k+1})\|$ in terms of the initial error $\|{\x}_{0} - \x^*(t_{0})\|$ and an extra error term for the bound of convergence. If we substitute $k+1$ by $k$ in \eqref{eq.rho_error_dependence} and recall the definition $\Gamma_2:= h\left(({2 C_0 L }/{m^2} )+ ({2 C_0 }/{m})\right)$ and $\Gamma:=(h^2/2)[(C_0 C_2)/(m^2) + (C_3/m)]$, then the result in \eqref{result2} follows.
%%
\qed

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%   S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem~\ref{th.NTT_convg} }\label{ap.newton}

We consider once again the proof of Theorem~\ref{th.GTT_convg}, in particular Equation~\eqref{some_bound} for $k = 0$, due to the prediction step. For the correction step, if we applied one time the Newton step, we would have that
\begin{equation}\label{eq.dummy300}
\|\x_{1} - \x^*(t_{1})\| \leq  (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \frac{\gamma C_1}{2 m} \|\x_{1|0} - \x^*(t_{1})\|^2.
\end{equation}
The reason for~\eqref{eq.dummy300} is explained as follows: Define
\begin{align}%\label{eq:thm1_defs2}
&\nabla_{\x\x}f_1 = \nabla_{\x\x}f(\x_{1|0}; t_1)\; , &&\nabla_{\x} f_1 = \nabla_{\x} f(\x_{1|0}; t_1)\;,\nonumber \\ 
&\nabla_{\x\x}f^*_1 = \nabla_{\x\x}f({\x}^*(t_{1}); t_1)\;,  && \nabla_{\x} f^*_1 = \nabla_{\x} f({\x}^*(t_{1}); t_{1}) \; . \nonumber
\end{align}
We can write, by applying one Newton step
\begin{align}
\|\x_{1} - \x^*(t_{1})\| &=  \|P_X[\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1]- \x^*(t_{1})\| \nonumber \\
& = \|P_X[\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1]- P_X[\x^*(t_{1})]\| \nonumber \\
& \leq \|\x_{1|0} - \gamma \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1- \x^*(t_{1})\|, \label{eq.aryan1}
\end{align}
where we have used the fact that $\x^*(t_{1}) \in X$ and the nonexpansive property of the projection. We can now expand the right-hand side of~\eqref{eq.aryan1} as
\begin{equation}\label{eq.aryan2}
(1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma\|\x_{1|0} - \x^*(t_{1}) - \nabla_{\x\x}f_1^{-1}\nabla_{\x}f_1\|,
\end{equation}
which can be further upper bounded as 
\begin{align}
\eqref{eq.aryan2} & \leq (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma\|\nabla_{\x\x}f_1^{-1}\|\times \nonumber \\ &\qquad\qquad\qquad\|\nabla_{\x\x}f_1(\x_{1|0} - \x^*(t_{1})) - \nabla_{\x}f_1\| \nonumber \\ 
&\leq (1-\gamma)\|\x_{1|0} - \x^*(t_{1})\| + \gamma \frac{C_1}{2 m}\| \x_{1|0} - \x^*(t_{1})\|^2,\label{eq.aryan3}
\end{align}

\textbf{Maybe expand this one!}

where the last inequality comes from the Assumption~\ref{as.smooth}, and in particular the Lipschitz continuity of the Hessian~[cfr.~\cite[Chapter~1]{Nesterov2004}]. By plugging the bound~\eqref{eq.aryan3} into~\eqref{eq.aryan1} the claim~\eqref{eq.dummy300} follows. 

Consider now $\gamma = 1$ and multiple Newton steps: we have,
\begin{equation}\label{eq.dummy30}
\|\x_{1} - \x^*(t_{1})\| \leq  \left(\frac{C_1}{2 m}\right)^{2\tau - 1}\hskip-2mm \left(\|\x_{1|0} - \x^*(t_{1})\|\right)^{2 \tau}.
\end{equation}
In order to ease the notation, we define $p_k$ as $\|\x_{k} - \x^*(t_{k})\|$ and $q = 2\tau -1$. By substituting~\eqref{eq.dummy30} into the bound on the predictions step~\eqref{some_bound}, we obtain, 
\begin{equation}\label{eq.dummy31}
p_1 \leq \left(\frac{C_1}{2 m}\right)^q  \left(\sigma p_0 + \|\mathbold{\Delta}\| \right)^{2\tau}.
\end{equation}
Due to strong convexity and Lipschitz continuity of the gradient (Assumptions~\ref{as.str} and \ref{as.smooth}), and the fact that at optimality the gradient vanishes, we can write
\begin{align}
\|\nabla_x f(\x_0, t_0)\| &= \|\nabla_x f(\x_0, t_0) - \nabla_x f^*_0\| \nonumber \\&\hspace*{-1.5cm}\geq (\nabla_x f(\x_0, t_0) - \nabla_x f^*_0)^\transp(\x_{0} - \x^*(t_0))/\|\x_{0} - \x^*(t_0)\| \nonumber \\  &\geq  m \|\x_{0} - \x^*(t_0)\|, 
\end{align}
\begin{equation}
\|\nabla_x f(\x_1, t_1)\| = \|\nabla_x f(\x_1, t_1) - \nabla_x f^*_1\| \leq L \|\x_{1} - \x^*(t_1)\|.
\end{equation}
Calling.. , due to , the inequality~\eqref{eq.dummy31} implies, 
\begin{equation}\label{eq.dummy31aryan}
g_1 \leq \frac{1}{L}\,\left(\frac{C_1}{2 m}\right)^q  \left(\sigma/m \,g_0 + \|\mathbold{\Delta}\| \right)^{2\tau}.
\end{equation}
and by recalling that by the local convergence hypothesis we have $g_0 \leq \beta\|\mathbold{\Delta}\|$, then
\begin{equation}\label{eq.dummy32}
g_1 \leq  \frac{1}{L} \left(\frac{C_1}{2 m}\right)^{q} \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau}.
\end{equation}

To enforce convergence of the sequence $\{g_k\}$, we need first to make sure that $g_1 \leq g_0$:
\begin{equation}\label{eq.dummy33}
\frac{1}{L}\left(\frac{C_1}{2 m}\right)^{q} \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau} \leq g_0 \leq \beta \|\mathbold{\Delta}\|,
\end{equation}
which yields
\begin{equation}\label{eq.dummy34}
\frac{C_1}{2 m}\|\mathbold{\Delta}\| \leq  \frac{(\beta\, L) ^{1/q}}{\left(\sigma/m\, \beta + 1 \right)^{2\tau/q}}.
\end{equation}
If condition~\eqref{eq.dummy34} is satisfied, then $g_1 \leq g_0$. By induction on $g_k$, one can show that under~\eqref{eq.dummy34}, it is also true that 
\begin{equation}\label{eq.dummy35}
g_k \leq \beta\,\|\mathbold{\Delta}\|, \quad \text{ for all } k\geq 1,
\end{equation}
or, by using again the strong convexity assumption
\begin{equation}\label{eq.dummy35}
p_k \leq g_k/m \leq \beta/m\,\|\mathbold{\Delta}\|, \quad \text{ for all } k\geq 1,
\end{equation}
which is the claim~\eqref{..}.

If we want to make sure to have a smaller asymptotical error (and quadratic convergence of the Newton method), then we need to change~\eqref{eq.dummy33} and enforce
\begin{equation}\label{eq.dummy36}
\frac{1}{L}\left(\frac{C_1}{2 m}\right)^{2\tau - 1}\hskip-2mm \|\mathbold{\Delta}\|^{2\tau} \left(\sigma/m\, \beta + 1 \right)^{2\tau} \leq \beta \|\mathbold{\Delta}\|^{2\tau}.
\end{equation}
Since $\|\mathbold{\Delta}\| \leq 1$ this condition is stronger than~\eqref{eq.dummy33} and implies $g_1 \leq g_0$. By solving~\eqref{eq.dummy36}, we obtain the condition:
\begin{equation}\label{eq.dummy37}
\left(\frac{C_1}{2 m}\right)^{q}  \leq \frac{\beta L}{\left(\sigma \beta + 1 \right)^{2\tau}},
\end{equation}
In particular, if this condition is satisfied then, 
\begin{equation}\label{eq.dummy38}
p_k \leq g_k/m \leq \beta/m \,\|\mathbold{\Delta}\|^{2\tau}, \quad \text{ for all } k\geq 1.
\end{equation}
%%%
which is . 
\qed


\section{Proof of Theorem~\ref{th.AGT_convg} }\label{ap.agt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     P  R   O  O   F    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We prove Theorem~\ref{th.AGT_convg} by evaluating the extra error term coming from the approximate time derivative in~\eqref{fobd}. In particular, by Taylor expansion, one can see that
\begin{equation}\label{appder_oh}
\|\tilde{\nabla}_{t\x}{f}_k  - {\nabla}_{t\x}{f}(\x_k; t_k)\| = O(h),  
\end{equation} 
In fact, one Taylor expands
\begin{align}
{\nabla}_{\x}{f}(\x_{k-1}; t_{k-1})  =& {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h \nonumber \\
& \quad + {\nabla}_{tt\x}{f}(\x(\tau); \tau) {h^2}/{2},
\end{align} 
for a particular choice of $\tau\in[t_{k-1}, t_k]$. By solving for ${\nabla}_{t\x}{f}(\x_k; t_k)$, 
\begin{align}
{\nabla}_{t\x}{f}(\x_k; t_k) = \frac{1}{h} ( {\nabla}_{\x}{f}(\x_k; t_k) - {\nabla}_{t\x}{f}(\x_k; t_k)\,h \nonumber \\
 + {\nabla}_{tt\x}{f}(\x(\tau); \tau) {h^2}/{2}).
\end{align}
By substituting this result and the definition~\eqref{fobd} into~\eqref{appder_oh}, the $O(h)$ error bound is proven. 

Consider now the approximate prediction step, 
\begin{equation}
\x_{k+1|k} = \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h,
\end{equation}
which by adding and subtracting the exact prediction direction becomes, 
\begin{align}
\x_{k+1|k} &= \x_k - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h + \nonumber \\ 
&\quad 
+[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} {\nabla}_{t\x}{f}(\x_k; t_k) \,h  \nonumber \\ 
&\quad - [{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1} \tilde{\nabla}_{t\x}{f}_k \,h.
\end{align}
By following the same steps as in Theorem~\ref{th.GTT_convg}, the term $a$ in Equation~\eqref{eq.hessian_cross_term} can be written with an extra error term as, 
\begin{align}\label{eq.hessian_cross_term_2}
a & \leq \left\|[\nabla_{\x\x}f]^{-1}\nabla_{t\x} f - [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f\right\|h \nonumber\\
 &\quad+  \left\| [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f- [\nabla_{\x\x}f^*]^{-1}\nabla_{t\x} f^*  \right\|h \nonumber \\ &\quad + \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h.
\end{align}
%
The extra error term w.r.t. Equation~\eqref{eq.hessian_cross_term} can be further bounded by using~\eqref{appder_oh} and the smoothness Assumption~\ref{as.smooth} (with the strong convexity constrant $m$)
\begin{align}\label{dummy_101}
& \|[{\nabla}_{\x\x}{f}]^{-1} {\nabla}_{t\x}{f} - [{\nabla}_{\x\x}{f}]^{-1} \tilde{\nabla}_{t\x}{f}_k \|\,h  \nonumber\\
&\quad \leq \|[{\nabla}_{\x\x}{f}(\x_k; t_k)]^{-1}\| \| {\nabla}_{t\x}{f}(\x_k; t_k)  - \tilde{\nabla}_{t\x}{f}_k \| \, h  \nonumber\\
&\quad \leq \frac{1}{m} \|{\nabla}_{tt\x}{f}(\x(\tau); \tau) {h}/{2}\| \, h = \frac{C_3}{m}\,\frac{h^2}{2}.
\end{align}
By adding this extra error term in the bounds~\eqref{some_bound} and \eqref{eq.a_subst} and proceeding in similar fashion as in the proof of Theorem~\ref{th.GTT_convg}, claims~\eqref{result2a} and \eqref{result1a} can be easily proven. 
%
\qed

\section{Proof of Theorem~\ref{th.ANT_convg} }\label{ap.ant}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%     P  R   O  O   F    %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The proof of Theorem~\ref{th.ANT_convg} is based on the proof of Theorems~\ref{th.NTT_convg} and \ref{th.AGT_convg}. In particular, the use of an approximate time derivative yields an additional error term equivalent to $({C_3}/{m})\,({h^2}/{2})$ as shown in~\eqref{dummy_101}. This means that~\eqref{eq.dummy31} will now read
\begin{align}
p_1 &\leq \left(\frac{C_1}{2 m}\right)^{q} \left(\sigma p_0 + \|\mathbold{\Delta}\| + \frac{C_3}{m}\,\frac{h^2}{2} \right)^{2\tau} \nonumber \\
 &= \left(\frac{C_1}{2 m}\right)^q (\sigma p_0 + D)^{2\tau} \; ,
\end{align}
where we have used the definition of the cumulative error $D$. The rest follows as in the proof of Theorem~\ref{th.NTT_convg}.
%
\qed

